Optimal Performance of Feedback Control Systems with Limited Communication over Noisy Channels

A discrete time stochastic feedback control system with a noisy communication channel between the sensor and the controller is considered. The sensor has limited memory. At each time, the sensor transmits encoded symbol over the channel and updates its memory. The controller receives a noisy version of the transmitted symbol, and generates a control action based on all its past observations and actions. This control action action is fed back into the system. At each stage the system incurs an instantaneous cost depending on the state of the plant and the control action. The objective is to choose encoding, memory updating and control strategies to minimize the expected total costs over a finite horizon, or the expected discounted cost over an infinite horizon, or the expected average cost per unit time over an infinite horizon. For each case we obtain a sequential decomposition of the optimization problem. The results are extended to the case when the sensor makes an imperfect observation of the state of the system.

==> discussion.tex <==
\section{An Alternative Formulation}\label{sec:alternate}

Consider the finite horizon problem of \autoref{sec:prob} for arbitrary (but fixed) encoder and memory update strategies. We seek to obtain the optimal control law. The system equations are given by
\begin{align}
  X_{t+1} &= f(X_t, U_t, W_t), \label{eq:alternative_a}\\
      M_t &= l_t(X_t, M_{t-1}), \\
      Z_t &= c_t(X_t, M_{t-1}), \\
      Y_t &= h_t(Z_t, N_t). \label{eq:alternative_b}
\end{align}
The instantaneous cost is given by $\rho(X_t,U_t)$. The variable $R_t \defined
(X_t, M_{t-1})$ can be considered as the state of the system and the
equations~\eqref{eq:alternative_a}--\eqref{eq:alternative_b} above can be
rewritten as
\begin{align}
  R_{t+1} &= \hat f_t (R_t, U_t, W_t), \label{eq:alternative_c}\\
      Y_t &= \hat h_t (R_t, N_t),      \label{eq:alternative_d}
\end{align}
with the instantaneous cost given by $\hat \rho(R_t, U_t) \defined \rho(X_t,
U_t)$. The objective is to choose a controller $g \defined (g_1,\dots,g_T)$ so
as to minimize
\begin{equation}
  \J(g) = \E{\sum_{t=1}^T \hat \rho(R_t, U_t) | g }. \label{eq:cost_again}
\end{equation}
Equations~\eqref{eq:alternative_c}--\eqref{eq:cost_again} is the canonical
form of a partial observation system.  The control laws can be defined in two
functional forms. The more commonly used form is
\begin{equation}
  U_t = g_t(Y_t, U^{t-1}). \label{eq:controller_a}
\end{equation}
An equivalent functional form $\hat g \defined (\hat g_1, \dots, \hat g_T)$
for the controller is 
\begin{align*}
  U_1 &= g_1(Y_1) \defined \hat g_1(Y_1), \\
  U_2 &= g_2\bigl(Y^2, g_1(Y_1) \bigr) \defined \hat g_2(Y^2), \\
  U_3 &= g_3\bigl(Y^3, g_2\bigl(Y^2, g_1(Y_1) \bigr) ,  g_1(Y_1) \bigr)
      \defined \hat g_3(Y^3),
\end{align*}
and so on. In general
\begin{equation}
  U_t = \hat g_t(Y^t) \label{eq:controller_b}.
\end{equation}
Both forms of the controller lead to a sequential decomposition of the
problem. In classical centralized stochastic optimization theory control laws
of the form~\eqref{eq:controller_a} are considered since they lead to a
parameter optimization problem, while control laws of the
form~\eqref{eq:controller_b} lead to a functional optimization problem. This
is because of the following reasons.

For control laws of the form~\eqref{eq:controller_a} an information state
sufficient for performance evaluation of the problem is given by
\begin{equation}
  \zeta_t \defined \Pr{R_t | Y^t, U^{t-1}, g^{t-1}}.
\end{equation}
This information state evolves as
\begin{equation}
  \zeta_{t+1} = F_t(\zeta_t, Y_{t+1}, U_t), \label{eq:evolution_a}
\end{equation}
where $F_t(\cdot)$ is a deterministic function. This information state leads
to a sequential decomposition of the problem given by: for all $\tilde
\zeta \in \P{\X\times\M}$,
\begin{gather}
  V_T(\tilde \zeta) = \min_{u_T \in \U} \E{\hat \rho(R_T, U_T) | \hat
  \zeta_T = \tilde \zeta, U_T}, \label{eq:alternative_DP_a_1} \\
  \intertext{and for $t = 1,2,\dots,T-1$}
  V_t(\tilde \zeta) = \min_{u_t \in \U} \E{\hat \rho(R_t, U_t) 
  + V_{t+1}\bigl(F_t(\zeta_t, Y_{t+1}, U_t)\bigr) | \hat
  \zeta_t = \tilde \zeta, U_t}. \label{eq:alternative_DP_a_2}
\end{gather}
Notice that the evolution of the information state given
by~\eqref{eq:evolution_a} does not depend on the control law~$g$. This results
in a Dynamic
program~\eqref{eq:alternative_DP_a_1}--\eqref{eq:alternative_DP_a_2} in which
the optimization problem at each step is a parameter optimization problem.

On the other hand, for control laws of the form~\eqref{eq:alternative_b} an
information state sufficient for performance evaluation is given by
\begin{equation}
  \hat \zeta_t \defined \Pr{R_t | Y^t, \hat g^{t-1}}
\end{equation}
This information state evolves as
\begin{equation} \label{eq:evolution_b}
  \hat \zeta_{t+1} = \widehat F_t(\hat \zeta_t, Y_{t+1}, \hat g_t),
\end{equation}
where $\widehat F_t(\cdot)$ is a deterministic function. This information
state leads to a sequential decomposition of the problem given by: for all
$\tilde \zeta \in \P{\X\times\M}$,
\begin{gather}
  V_T(\tilde \zeta) = \inf_{\hat g_T \in \sG} \E{\hat \rho(R_T, U_T) | \hat
  \zeta_T = \tilde \zeta, \hat g_T}, \label{eq:alternative_DP_b_1} \\
  \intertext{and for $t = 1,2,\dots,T-1$}
  V_t(\tilde \zeta) = \inf_{\hat g_t \in \sG} \E{\hat \rho(R_t, U_T) 
  + V_{t+1}\bigl(F_t(\zeta_t, Y_{t+1}, \hat g_t)\bigr) | \hat
  \zeta_t = \tilde \zeta, \hat g_t}. \label{eq:alternative_DP_b_2}
\end{gather}
Notice that the evolution of the information state given
by~\eqref{eq:evolution_b} depends on the control law~$\hat g$. This results in
a Dynamic program~\eqref{eq:alternative_DP_b_1}--\eqref{eq:alternative_DP_b_2}
in which the optimization problem at each step is a functional optimization
problem.

Parameter optimization problems are easier to solve than functional
optimization problems. For this reason, in classical centralized stochastic
control theory, control laws of the form~\eqref{eq:controller_a} are
preferred over control laws of the form~\eqref{eq:controller_b}. The problem
considered in this paper is, however, a decentralized stochastic optimization
problem with strictly non-classical information structure. The joint
optimization problem is a functional optimization problem and no choice of
information state will transform it into a parameter optimization problem.
Thus for the paper considered in this paper, there is no disadvantage of
choosing control laws of the form~\eqref{eq:controller_b}. Even if the model
of \autoref{sec:prob} was defined with control law of the
form~\eqref{eq:controller_b}, we can obtain a sequential decomposition alogn
the lines of the original problem.
The definition of
the beliefs of the controllers (\autoref{def:beliefs}) needs to be changed as
follows.
\begin{definition}
  Let \hPXM tt, \hPXM {t+1}t and \hPXMp {t+1}t be random vectors defined as 
  follows:
  \begin{enumerate}
    \item $\hPXM tt(x,m) = \Pr{ X_t = x, M_t = m | Y^t, c^t, l^t, 
      \hat g^{t-1}}$.
    \item $\hPXM {t+1}t(x,m) = \Pr{ X_{t+1} = x, M_t = m | Y^t, c^t, l^t, 
      \hat g^t}$.
    \item $\hPXMp{t+1}t(x,m) = \Pr{ X_{t+1} = x, M_t = m | Y^{t+1}, 
      c^{t+1}, l^t, \hat g^t}$.
  \end{enumerate}
\end{definition}
These beliefs are related to each other as in \autoref{lemma:beliefs}
with~\eqref{eq:psi} replaced by
\begin{equation}
  \hPXM {t+1}t = \psi( \hPXM tt, \hat g_t ).
\end{equation}
With these modified definition of the beliefs of the controller we can
establish the structural results---{\itshape without loss of optimality, we
can restrict attention to control laws of the form}
\begin{equation}
  U_t = \hat g_t(\hPXM tt).
\end{equation}
This can be proved along the lines of the proof of \autoref{thm:structural}.
For a given encoder and memory update strategies, the optimal control
strategies of the above structural form can only be obtained using a Dynamic
program where each step is a functional optimization problem. But we are not
interested in finding the optimal control strategy for a given encoder and
memory update strategies. We are interested in the joint optimization of
encoder, memory update and control strategies. For the joint optimization
problem, control laws of the form~\eqref{eq:controller_a}
and~\eqref{eq:controller_b} both lead to a Dynamic program in which each step
is a functional optimization problem. As such, there is no inherent advantage
of considering control laws of the form~\eqref{eq:controller_a}. If we start
with control laws of the form~\eqref{eq:controller_b}, the nested optimality
equations~\eqref{eq:DPbasic}--\eqref{eq:DPn} may be easier to solve
numerically when the state space is uncountable.



\section{Comparison with real-time communication problems} \label{sec:comm}
Real-time communication problems are a special case of the control problem
described in this paper. Suppose the feedback link is absent, so that the
control action does not affect the evolution of the system, i.e.,
\begin{equation}
  X_{t+1} = f_t(X_t, U_t, W_t) = \hat f_t(X_t, W_t)
\end{equation}
For this particular plant function, the control problem described in this
paper is equivalent to a real-time communication problem; the plant models a
Markovian source\footnote{The process $\{X_1, X_2, \dots, X_T\}$ is Markovian
because $W_1,\dots, W_T$ are independent random variables and are also
independent of $X_1$.} with known statistics\footnote{The statistics of the
source can be obtained by using the plant functions $\hat f_1, \dots, \hat
f_T$ and the statistics of $W_1, \dots, W_T$.}, and the sensor models a
real-time finite-memory encoder for the source. The channel given
by~\eqref{eq:channel} is a discrete memoryless channel.  The control action
does not affect the evolution of the system and can be thought of as a
real-time decoder of the source. The control action $U_t$ can be considered as
an estimate of the source output $X_t$ at time $t$. The cost $\rho(X_t, U_t)$
can be interpreted as the distortion of reconstruction.  The objective is to
choose real-time encoding, memory updating and real-time decoding strategies
minimize the expected total distortion over a finite horizon.

The methodology presented in this paper can be used to obtain optimal encoders
and decoders for real-time communication problems. This methodology is similar
in spirit to the approach taken
in~\cite{Witsenhausen:1978,WalrandVaraiya:1983,Teneketzis:2006} to obtain
structural results for optimal encoders and decoders and the approach taken
in~\cite{MahajanTeneketzis:2005a,MahajanTeneketzis:2006,MahajanTeneketzis:2006a}
to obtain jointly optimal real-time encoder/decoder for joint source-channel
coding for Markovian sources. 

\section{Relation to Witsenhausen's Counterexample}\label{sec:Wit}

The methodology presented in this paper applies to general sequential
stochastic optimization problems with non-classical information structures.
To illustrate how to use this methodology in a general problem, we consider
the classical problem referred to as the \emph{``Witsenhausen
counterexample''}~\cite{Witsenhausen:1968}.

Many results of classical stochastic optimization theory hold only for
problems with classical information structure. For example, for the
unconstrained  control of linear systems with Gaussian noise and quadratic
criteria (called the \textsc{lqg} problem), when the information structure is
classical, we can restrict attention to affine control laws without any loss
of optimality. However for non-classical information structures, restricting
attention the class of affine functions is not always adequate for
optimization. Witsenhausen considered a simple two stage \textsc{lqg} problem
with non-classical information structure and showed that non-linear control
laws outperform the best affine control laws~\cite{Witsenhausen:1968}. He also obtained a sequential
decomposition of the problem by an insight on the special structure of the
``counterexample.'' We show how the methodology presented in this paper can
be used to obtain a sequential decomposition of the Witsenhausen
counterexample.

We formulate a problem identical to the Witsenhausen counterexample. We do not
restrict ourselves to linear systems, Gaussian noise or quadratic cost since,
in light of Witsenhausen's result, these restrictions do not simplify the
analysis. For ease of exposition, we assume that all random variables take
values in a finite set. Consider the following two stage partial observation
system:
\begin{align}
  Y_1 &= h_1(X_1, N_1),\label{eq:W1} \\
  U_1 &= g_1(Y_1)     ,\\
  X_2 &= f_1(X_1, U_1),\\
  Y_2 &= h_2(X_2, N_2),\\
  U_2 &= g_2(Y_2),\label{eq:W5}
\end{align}
where for $t=1,2$, $X_t$ represents the state of the system and takes values
in $\X \defined \{1,\dots,\abs\X\}$, $Y_t$ represents the observations of the
controller and takes values in $\Y \defined \{1,\dots,\abs\Y\}$, $U_t$
represents the control action and takes values in $\U \defined \{1,\dots,
\abs\U\}$, and $N_t$ represents the observation noise and takes values in $\N
\defined \{1,\dots,\abs\N\}$. The variables $X_1$, $N_1$, $N_2$ are
independent random variables with known distributions. At each stage $t$,
$t=1,2$, the system incurs an instantaneous cost $\rho_t(X_t, U_t)$, where
$\rho_t : \X \times \U \to [0,\infty)$. The choice of $g_1$, $g_2$ is called a
design. Performance of a design is quantified by the expected total cost under
that design, which is given by
\begin{equation}
  \J(g_1, g_2) = \E{\rho_1(X_1, U_1) + \rho_2(X_2, U_2) | g_1, g_2 },
\end{equation}
where the expectation is with respect to a joint measure on $(X_1, X_2, U_1,
U_2)$ determined by the measure on $(X_1, N_1, N_2)$, the channel functions
$h_1$, $h_2$ and the choice of control laws $g_1$, $g_2$.

The optimization problem under consideration is the following:
\begin{problem}\label{prob:witsenhausen}
  Consider the partial observation system \eqref{eq:W1}--\eqref{eq:W5}. Given
  $(\X,\allowbreak \Y,\allowbreak \U,\allowbreak \N, \allowbreak h_1,
  \allowbreak h_2)$ and measure on $(X_1,N_1,N_2)$ determine an optimal
  design $(g_1^*, g_2^*)$ such that,
  \begin{equation}
    \J(g_1^*,g_2^*) = \J^* \defined \min_{(g_1,g_2) \in \sG^2} \J(g_1,g_2),
  \end{equation}
  where $\sG$ is the family of functions from $\Y$ to $\U$.
\end{problem}

\autoref{prob:witsenhausen} is the simplest problems with non-classical
information structure. To obtain a sequential decomposition for the problem we
consider the following:

\begin{definition}\label{def:witsenhausen}
  Let $\pi_1$, $\pi_2$ be random vectors given by
  \begin{align}
    \pi_1(x) &= \Pr{X_1 = x} \\
    \pi_2(x) &= \Pr{X_2 = x}
  \end{align}
\end{definition}

The random vectors $\pi_1$ and $\pi_2$ are information states sufficient for
performance evaluation. Specifically, they satisfy the following properties.

\begin{lemma}\label{lemma:witsenhausen}
  \begin{enumerate}
    \item There exists a linear transformation $Q(g_1)$ such that
      \begin{equation}\label{eq:Wtransformation}
        \pi_2 = Q(g_1)\pi_1
      \end{equation}
    \item For $t=1,2$, the expected instantaneous cost at $t$ can be expressed
      as
      \begin{equation}
        \E{\rho_t(X_t,U_t) | g_1, g_2} = \hat \rho_t(\pi_t, g_t),
      \end{equation}
      where $\hat \pi$ is a deterministic function.
  \end{enumerate}
\end{lemma}
\begin{proof}
  \begin{enumerate}
    \item The belief $\pi_2$ can be decomposed as follows:
      \begin{equation} \begin{split}
        \pi_2 &= P(X_2) = \bigvee_{X_1,N_1} P(X_2, N_1, X_1) \\
        &= \bigvee_{X_1,N_1} P\bigl(X_2 \bigm| g_1\bigl(h_1(X_1,N_1)\bigr)
        \bigr) P(X_1)P(N_1) \\
        & \defined Q(g_1) \pi_1,
      \end{split} \end{equation}
      where $\bigvee_X$ denotes marginalization of the joint density with
      respect to $X$.
    \item The expected instantaneous cost can be simplified as follows:
      \begin{equation} \begin{split}
        \E{\rho_t(X_t, U_t) | g_1, g_2} &=
          \sum_{X_t, N_t} \rho_t\bigl(X_t, g_t\bigl(h_t(X_t, N_t)\bigr)\bigr)
          P(X_t)P(N_t) \\
          &\defined \hat \rho_t (\pi_t, g_t).
        \end{split} \end{equation}
    \end{enumerate}
\end{proof}

Using the above properties, we can reduce \autoref{prob:witsenhausen} to a
deterministic system with state $\pi_t$ which evolves according
to~\eqref{eq:Wtransformation} and incurs instantaneous cost $\hat \rho(\pi_t,
g_t)$. A sequential decomposition for this equivalent deterministic problem is
given by
\begin{align}
  V_2(\pi_2) &= \min_{g_2 \in \sG} \hat \rho_2(\pi_2, g_2), \label{eq:Wseq1} \\
  V_1(\pi_1) &= \min_{g_1 \in \sG} \hat \rho_1(\pi_1, g_1) +
  V_2\bigl(Q(g_1)\pi_1\bigr). \label{eq:Wseq2}
\end{align}

The sequential decomposition given above is also valid if $\X$, $\Y$, $\U$,
$\N$, are not finite spaces. Suppose $\X = \Y = \U = \N = \RR$ and 
\begin{align}
  f_1(X_1, U_1) & \defined X_1 + U_1 ,\\
  h_1(X_1, N_1) & \defined X_1, \\
  h_2(X_2, N_2) & \defined X_2 + N_2, \\
  \rho_1(X_1, U_1) & \defined K^2 U_1^2 ,\\
  \rho_2(X_2, U_2) & \defined (X_2 - U_2)^2. 
\end{align}
Under these assumptions the model of~\eqref{eq:W1}--\eqref{eq:W5} is
equivalent to the model of the counterexample in~\cite{Witsenhausen:1968}.

The sequential decomposition of~\eqref{eq:Wseq1}--\eqref{eq:Wseq2} can be
simplified as
\begin{equation} \begin{split}
  V_2(\pi_2) &= \min_{g_2 \in \sG} \E{ \rho_2(X_2, U_2) | P_{X_2}, g_2} \\
  &= \min_{g_2 \in \sG} \E{ \bigl(X_2 - g_2(X_2 + N_2) \bigr)^2 | P_{X_2},
  g_2}.
\end{split} \end{equation}

From filtration theory \textbf{add a reference} we know that the optimal
$g_2$ is given by the conditional expectation of $X_2$, i.e.,
\begin{equation} \label{eq:Wcond}
  g_2^*(Y_2) = \E{X_2 | Y_2},
\end{equation}
and
\begin{equation} \label{eq:WV2}
  V_2(\pi_2) = \E{ \mathop{\text{Var}}(X_2 \mid Y_2) },
\end{equation}
where the outer expectation is with respect to the measure $\pi_2$ on $X_2$.

This corresponds to Lemma~3 of~\cite{Witsenhausen:1968}. Witsenhausen further
simplified~\eqref{eq:Wcond} and~\eqref{eq:WV2} to obtain closed form
expression for $g_2$ and $V_2$ in terms of $g_1$ and $\pi_1$.

Simplifying $V_1$ is much harder because $\hat \rho_1(\pi_1, g_1) +
V_2\bigl(Q(g_1)\pi_1\bigr)$ is not convex in $g_1$. Witsenhausen identified
many structural properties of the minimizer which helps in restricting the
set of functions that need to be searched for a minimizer. However, due to the
non-convex nature of the objective, usual computation methods like gradient
decent can not be used. Researchers have identified other techniques to obtain
the minima numerically~\cite{LeeLauHo:2001,BagliettoParisiniZoppoli:2001}. Computational techniques for
these type of non-convex functional optimization problems need further
investigation.


==> figures.tex <==
\empprelude{input mp-tool;^^Jinput metaobj}
\begin{empfile}
  \begin{empcmds}
    % Default Options
    setObjectDefaultOption("Box")("dx")(10pt);
    setObjectDefaultOption("Box")("dy")(10pt);
    %     setObjectDefaultOption("Box")("shadow")(true);
    setObjectDefaultOption("Box")("framewidth")(1bp);
    setObjectDefaultOption("Box")("filled")(true);
    setObjectDefaultOption("Box")("fillcolor")(0.9white);

    setObjectDefaultOption("HBox")("hbsep")(1cm);
    setObjectDefaultOption("HBox")("align")("center");

    setCurveDefaultOption("linewidth",1bp);
  \end{empcmds}
  \begin{empdef}[feedback](4,2.5)
    newRBox.plant(btex System etex) ;
    newRBox.encoder(btex Encoder etex) ;
    newRBox.memory(btex Memory etex) ;
    newCircle.channel(btex \Huge $\times$ etex) ;
    newEmptyBox.channel_label(1bp,1bp) ;
    newRBox.controller(btex Controller etex);
    newMatrix.sensor(2,2)(nb,encoder,memory,nb) "hsep(1.2cm)", "vsep(0.8cm)",
    "framed(true)", "framestyle(dashed evenly)", "dx(10pt)", "dy(10pt)" ;

    newHBox.temp1(plant,encoder) "hbsep(5cm)";
    newVBox.temp2(controller,temp1) "vbsep(3cm)", "align(center)" ;
    newHBox.temp3(temp2,channel) ;
    plant.c = origin ;
    drawObj(plant,sensor,channel,controller);

    ncline(plant)(encoder) ;
    ncangle(encoder)(channel) "angleA(0)", "angleB(90)";
    ncangle(channel)(controller) "angleA(90)", "angleB(0)" ;
    ncangle(plant)(memory) "angleA(0)", "angleB(-90)" ;
    ncangle(memory)(encoder) "angleA(0)", "angleB(90)";
    ncangle(controller)(plant) "angleA(180)", "angleB(90)";
    drawarrow (channel.e + (1cm,0))--(channel.e) ;

    label.top(btex $X_t$ etex, 0.2[plant.e,encoder.w]) ;
    label.top(btex $M_{t-1}$ etex, 0.5[memory.e, (xpart encoder.s, ypart
    memory.e) ] );
    label.top(btex $Z_t$ etex, encoder.e + (1cm,0)) ;
    label.top(btex $Y_t$ etex, controller.e + (1cm,0)) ;
    label.top(btex $U_t$ etex, controller.w - (1cm, 0) ) ;
    label.bot(btex Sensor etex, sensor.s) ;
    label.rt(btex $N_t$ etex, channel.e + (1cm,0)) ;
  \end{empdef}
  \begin{empdef}[imperfect](4,2.5)
    % Reset all previous relations
    untieObj(sensor) ;
    untieObj(plant) ;
    untieObj(channel) ;
    untieObj(controller) ;
    newCircle.obs_channel(btex \Huge $\times$ etex) ;
    newEmptyBox.obs_channel_label(1bp,1bp) ;
    newHBox.temp11(plant,encoder) "hbsep(6cm)";
    plant.c - obs_channel.c = -(2cm,0) ;
%    newHBox.temp21(temp11,encoder) "hbsep(5cm)";
    newVBox.temp12(controller,temp11) "vbsep(3cm)", "align(center)" ;
    newHBox.temp13(temp12,channel) ;
    plant.c = origin ;
    drawObj(plant,sensor,obs_channel,channel,controller) ;

    ncline(plant)(obs_channel) ;
    ncline(obs_channel)(encoder) ;
    ncangle(encoder)(channel) "angleA(0)", "angleB(90)";
    ncangle(channel)(controller) "angleA(90)", "angleB(0)" ;
    ncangle(obs_channel)(memory) "angleA(0)", "angleB(-90)" ;
    ncangle(memory)(encoder) "angleA(0)", "angleB(90)";
    ncangle(controller)(plant) "angleA(180)", "angleB(90)";
    drawarrow (channel.e + (1cm,0))--(channel.e) ;
    drawarrow (obs_channel.n + (0,1cm))--(obs_channel.n) ;

    label.top(btex $X_t$ etex, 0.5[plant.e,obs_channel.w]) ;
    label.top(btex $S_t$ etex, 0.2[obs_channel.e,encoder.w]) ;
    label.top(btex $M_{t-1}$ etex, 0.5[memory.e, (xpart encoder.s, ypart
    memory.e) ] );
    label.top(btex $Z_t$ etex, encoder.e + (1cm,0)) ;
    label.top(btex $Y_t$ etex, controller.e + (1cm,0)) ;
    label.top(btex $U_t$ etex, controller.w - (1cm, 0) ) ;
    label.bot(btex Sensor etex, sensor.s) ;
    label.rt(btex $N_t$ etex, channel.e + (1cm,0)) ;
    label.top(btex $\widehat N_t$ etex, obs_channel.n + (0,1cm)) ;
  \end{empdef}
  \begin{empdef}[timing](4,2.5)
      numeric hsep ; hsep := 4cm ;
      numeric arrow ; arrow := 1cm ;
      numeric e ; e := 2mm ;
      numeric dy ; dy = 1.3cm ;
      pair t[], t_half[] ;
      t[0] := origin ;
      t[1] := t[0] + (hsep, 0) ;
      t[2] := t[1] + (hsep, 0) ;
      t_half[1] := 0.5[ t[0], t[1] ] ;
      t_half[2] := 0.5[ t[1], t[2] ] ;
      drawarrow (t[0]-(hsep/2,0))--(t[2]+(hsep/2,0)) withpen pencircle scaled 
      1bp ;
      for pts = t[0], t[1], t[2], t_half[1], t_half[2]:
        draw (xpart pts, ypart pts + dy)--(xpart pts, ypart pts -dy) dashed 
        evenly;
      endfor ;
      for pts = t[0], t[1], t[2] :
        drawarrow (xpart pts - e, ypart pts - arrow)--(pts-(e,0)) ;
        drawarrow (xpart pts + e, ypart pts - arrow)--(pts+(e,0)) ;
      endfor
      for pts = t_half[1], t_half[2] :
        drawarrow (xpart pts , ypart pts - arrow)--pts ;
      endfor
      label.rt(btex $t$ etex, t[2] + (hsep/2,0) ) ;
      label.top(btex $t$ etex, t[0] + (0,dy) ) ;
      label.top(btex $t+1$ etex, t[1]  + (0,dy) ) ;
      label.top(btex $t+2$ etex, t[2]  + (0,dy) ) ;
      label.top(btex $t + \frac12$ etex, t_half[1]  + (0,dy) ) ;
      label.top(btex $t + \frac32$ etex, t_half[2]  + (0,dy) ) ;
      label.llft(btex $g_{t-1}$ etex, t[0] - (e,arrow) ) ;
      label.llft(btex $g_{t}$ etex,   t[1] - (e,arrow) ) ;
      label.llft(btex $g_{t+1}$ etex, t[2] - (e,arrow) ) ;
      label.lrt(btex $c_{t}$ etex, t[0] + (e,-arrow) ) ;
      label.lrt(btex $c_{t+1}$ etex, t[1] + (e,-arrow) ) ;
      label.lrt(btex $c_{t+2}$ etex, t[2] + (e,-arrow) ) ;
      label.lrt(btex $l_t$ etex, t_half[1] - (0,arrow) ) ;
      label.lrt(btex $l_{t+1}$ etex, t_half[2] - (0,arrow) ) ;
  \end{empdef}
  \begin{empdef}[decisions](4,2.5)
      numeric hsep ; hsep := 8cm ;
      numeric arrow ; arrow := 1cm ;
      numeric e ; e := 2mm ;
      numeric dy ; dy = 1.3cm ;
      pair t[], t_half[] ;
      t[0] := origin ;
      t[1] := t[0] + (hsep, 0) ;
      t[2] := t[1] + (hsep, 0) ;
      t_half[1] := 0.5[ t[0], t[1] ] ;
      t_half[2] := 0.5[ t[1], t[2] ] ;
      drawarrow (t[0]-(hsep/2,0))--(t[1]+(hsep/2,0)) withpen pencircle scaled 
      1bp ;
%      for pts = t[0], t[1], t[2], t_half[1], t_half[2]:
      for pts = t[0], t[1], t_half[1],:
        draw (xpart pts, ypart pts + dy)--(xpart pts, ypart pts -dy) dashed 
        evenly;
      endfor ;
%      for pts = t[0], t[1], t[2] :
      for pts = t[0], t[1]:
        drawarrow (xpart pts - e, ypart pts - arrow)--(pts-(e,0)) ;
        drawarrow (xpart pts + e, ypart pts - arrow)--(pts+(e,0)) ;
        drawarrow (pts-(1.5e,0))--(xpart pts -1.5*e, ypart pts + arrow) ;
        drawarrow (pts+(e/2,0))--(xpart pts +e/2, ypart pts + arrow) ;
      endfor
%      for pts = t_half[1], t_half[2] :
      for pts = t_half[1] :
        drawarrow (xpart pts , ypart pts - arrow)--pts ;
        drawarrow (pts-(.5e,0))--(xpart pts - .5e, ypart pts + arrow) ;
      endfor
      label.rt(btex $t$ etex, t[1] + (hsep/2,0) ) ;
      label.top(btex $t$ etex, t[0] + (0,dy) ) ;
      label.top(btex $t+1$ etex, t[1]  + (0,dy) ) ;
      label.top(btex $t+2$ etex, t[2]  + (0,dy) ) ;
      label.top(btex $t + \frac12$ etex, t_half[1]  + (0,dy) ) ;
%      label.top(btex $t + \frac32$ etex, t_half[2]  + (0,dy) ) ;
      label.llft(btex $g_{t-1}$ etex, t[0] - (e,arrow) ) ;
      label.llft(btex $g_{t}$ etex,   t[1] - (e,arrow) ) ;
%      label.llft(btex $g_{t+1}$ etex, t[2] - (e,arrow) ) ;
      label.lrt(btex $c_{t}$ etex, t[0] + (e,-arrow) ) ;
      label.lrt(btex $c_{t+1}$ etex, t[1] + (e,-arrow) ) ;
%      label.lrt(btex $c_{t+2}$ etex, t[2] + (e,-arrow) ) ;
      label.lrt(btex $l_t$ etex, t_half[1] - (0,arrow) ) ;
%      label.lrt(btex $l_{t+1}$ etex, t_half[2] - (0,arrow) ) ;
      label.lft(btex \small $\widetilde P_{X_{t-1},M_{t-1}}$ etex,
                 t[0] + (-1.5e,arrow) ) ;
      label.lft(btex \small $\widetilde P_{X_{t},M_{t}}$ etex,
                 t[1] + (-1.5e,arrow) ) ;
%      label.lft(btex \small $\widetilde P_{X_{t+1},M_{t+1}}$ etex,
%                 t[2] + (-1.5e,arrow) ) ;
      label.rt(btex \small $\widetilde P_{X_t,M_{t-1}}$ etex,
                 t[0] + (.5e, arrow) ) ;
      label.rt(btex \small $\widetilde P_{X_{t+1},M_{t}}$ etex,
                 t[1] + (.5e, arrow) ) ;
%      label.rt(btex \small $\widetilde P_{X_{t+2},M_{t+1}}$ etex,
%                 t[2] + (.5e, arrow) ) ;
      label.lft(btex \small $\widetilde P^+_{X_t,M_{t-1}}$ etex,
                t_half[1] + (-.5e,arrow) );
%      label.lft(btex \small $\widetilde P^+_{X_{t+1},M_{t}}$ etex,
%                t_half[2] + (-.5e,arrow) );
  \end{empdef}
\end{empfile}
\ifProcessMP
\immediate\write18{mp -tex=latex \jobname.mp}
\fi

\endinput
  \begin{empdef}[2controllers](4,2.5)
    newRBox.plant1(btex System etex) ;
    newRBox.sensor11(btex Sensor 1 etex) ;
    newRBox.sensor12(btex Sensor 2 etex) ;
    newRBox.controller11(btex Controller 1 etex) ;
    newRBox.controller12(btex Controller 2 etex) ;
    newCircle.channel11(btex \Huge $\times$ etex) ;
    newCircle.channel12(btex \Huge $\times$ etex) ;

    newHBox.temp11(sensor11, channel11) "hbsep(3cm)" ;
    newHBox.temp12(sensor12, channel12) "hbsep(3cm)" ;
    newVBox.temp13(temp12, temp11) "vbsep(2cm)" ;
    newVBox.temp14(controller11, controller12, temp13) "vbsep(2cm)", "align(center)" ;
    newHBox.temp15(plant1, temp13) "hbsep(3cm)" ; 

    plant1.c = origin
    drawObj(plant1,sensor11,sensor12, controller11, controller12, channel11,
    channel12) ;

    ncline(plant1)(sensor11) ;
    ncline(plant1)(sensor12) ;
    ncline(sensor11)(channel11) ;
    ncline(sensor12)(channel12) ;
    ncbar(channel11)(controller11) "angleA(0)", "armA(4cm)";
    ncbar(channel12)(controller12) "angleA(0)" , "armA(2cm)";

    ncangle(controller11)(plant1) "angleA(0)", "angleB(0)" ;
    ncangle(controller12)(plant1) "angleA(0)", "angleB(90)" ;

    drawarrow (channel11.n + (0,1cm))--(channel11.n) ;
    drawarrow (channel12.n + (0,1cm))--(channel12.n) ;

    label.lft(btex $S_{1,t}$ etex, sensor11.w ) ;
    label.lft(btex $S_{2,t}$ etex, sensor12.w ) ;
    label.urt(btex $Z_{1,t}$ etex, sensor11.e  + (1cm,0)) ;
    label.urt(btex $Z_{2,t}$ etex, sensor12.e + (1cm,0) ) ;
    label.top(btex $N_{1,t}$ etex, channel11.n + (0,1cm) ) ;
    label.top(btex $N_{2,t}$ etex, channel12.n + (0,1cm) ) ;
    label.top(btex $Y_{1,t}$ etex, controller11.e + (1cm,0) ) ;
    label.top(btex $Y_{2,t}$ etex, controller12.e + (1cm,0) ) ;
    label.top(btex $U_{1,t}$ etex, controller11.w - (1cm,0) ) ;
    label.top(btex $U_{2,t}$ etex, controller12.w - (1cm,0) ) ;
    label.top(btex $X_t$ etex, plant1.n ) ;
   
   \end{empdef}
  \begin{empdef}[1controller](4,2.5)
    newRBox.plant2(btex System etex) ;
    newRBox.sensor21(btex Sensor 1 etex) ;
    newRBox.sensor22(btex Sensor 2 etex) ;
    newRBox.controller2(btex Controller etex) ;
    newCircle.channel21(btex \Huge $\times$ etex) ;
    newCircle.channel22(btex \Huge $\times$ etex) ;

    newHBox.temp21(sensor21, channel21) "hbsep(5cm)" ;
    newHBox.temp22(sensor22, channel22) "hbsep(5cm)" ;
    newVBox.temp23(temp22, temp21) "vbsep(2cm)" ;
    newVBox.temp24(controller2, temp23) "vbsep(2cm)", "align(center)" ;
    newHBox.temp25(plant2, temp23) "hbsep(3cm)" ; 

    plant2.c = origin
    drawObj(plant2,sensor21,sensor22, controller2, channel21, channel22) ;

    ncline(plant2)(sensor21) ;
    ncline(plant2)(sensor22) ;
    ncline(sensor21)(channel21) ;
    ncline(sensor22)(channel22) ;
    ncbar(channel21)(controller2) "angleA(0)", "armA(4cm)";
    ncangles(channel22)(controller2) "angleA(0)" ,"angleB(-30)", "armA(2cm)";

    ncangle(controller2)(plant2) "angleA(0)", "angleB(0)" ;

    drawarrow (channel21.n + (0,1cm))--(channel21.n) ;
    drawarrow (channel22.n + (0,1cm))--(channel22.n) ;
  \end{empdef}


% vim: syntax=mp


==> uncountable_space.tex <==
\section{Uncountable State Space}
\label{sec:uncountable}

Consider the model of \autoref{sec:prob} with the following differences: the
state of the plant $X_t$, the plant disturbance $W_t$ and the control action
$U_t$ belong to uncountable spaces, i.e., $\X = \RR^{d_X}$, $\W = \RR^{d_W}$
and $\U = \RR^{d_U}$ where $d_X$, $d_W$ and $d_U$ are positive integers. The
initial state $X_1$ is a random variable belonging to $(\RR^{d_X},
\BOREL{\RR^{d_X}}, \mu_{X_1})$, where $\BOREL{\RR^{d_X}}$ is the Borel
$\sigma$-algebra on $\RR^{d_X}$ and the probability law $\mu_{X_1}$ is given.
The plant disturbance $W_1, \dots, W_T$ are i.i.d.\ random variables belonging
to $(\RR^{d_W}, \BOREL{\RR^{d_W}}, \mu_W)$ where the probability law $\mu_W$
is given. The conditional probability $\Pr{X_{t+1} \in A | X_t }$, $A \in
\BOREL{\RR^{d_X}}$, which represents the transition probability of the source,
is given. The rest of the model is the same as the model of
\autoref{sec:prob}. The sensor has finite memory $\M$ and the channel is a
discrete memoryless channel with input $\Z$ and output $\Y$. The plant
function $f$, the design $(\design)$, $c \defined (c_1, \dots, c_T)$, $g
\defined (g_1, \dots, g_T)$, $l \defined (l_1, \dots, l_T)$ and the cost
$\rho$ are Borel measurable with respect to appropriate $\sigma$-algebras. The
objective is to choose a design $(\design)$ that minimizes the total expected
cost under that design.

The fact that the state of the plant, the plant disturbance, and the control
action belong to uncountable spaces does not change the problem fundamentally.
The  methodology of finite state space applies here---the technical details
are a bit more involved.

\subsection{Structural Results}
For a fixed encoder, the design of optimal encoder is a \pomdp as in
the case of finite state space. We need to modify the definition of beliefs,
given by \autoref{def:beliefs}, to take  the uncountable state
space into account.
\begin{definition}\label{def:beliefs_uncountable}
  For any $A \in \BOREL{\RR^{d_X}}$, $B \in 2^{\M}$, where $2^{\M}$ denotes
  the power set of $\M$, define the measurable transforms \PXM tt, \PXM {t+1}t
  and \PXMp {t+1}t as follows: 
  \begin{enumerate}
    \item $\PXM tt(A,B) = \Pr{ X_t \in A, M_t \in B | Y^t, U^{t-1}, c^t, l^t, 
      g^{t-1}}$.
    \item $\PXM {t+1}t(A,B) = \Pr{ X_{t+1} \in A, M_t \in B | Y^t, U^t, c^t, l^t, 
      g^t}$.
    \item $\PXMp{t+1}t(A,B) = \Pr{ X_{t+1} \in A, M_t \in B | Y^{t+1}, U^t, 
      c^{t+1}, l^t, g^t}$.
  \end{enumerate}
\end{definition}
For any particular realization $y^t, u^{t-1}$ and arbitrary (but fixed) 
choice of $c^t$, $l^{t}$ and $g^{t-1}$, the realization of \PXM tt, denoted 
by \tPXM tt is a probability measure on $\bigl(\RR^{d_X} \times \M,
\BOREL{\BOREL{\RR^{d_X}}\times2^{\M}}\bigr)$. If $(Y^t, U^{t-1})$ is a random
vector and $c^t, l^{t}, g^{t-1}$ are arbitrary (but fixed) functions, then
\PXM tt is a version of conditional probability on $(\RR^{d_X} \times \M,
\BOREL{\RR^{d_X}}\times2^{\M})$. \PXM tt belongs to $\P{\X\times\M}$, the
Borel space of PMFs on $\X\times\M$.  Similar interpretations hold for \PXM
{t+1}t and \PXM {t+1}t.

\autoref{lemma:beliefs} can be proved as before by using Bayes rule
for continuous valued random variables. \autoref{lemma:beliefs} implies that  \autoref{thm:structural} also holds in
this case. Instead of a \pomdp where the unobservable state is finite, we have
a \pomdp where the unobservable state is uncountable. The Markov decision
theory arguments hold for this case also (see~\cite[Chater~8.4]{Dynkin:1975}).
Thus without loss of optimality, we can restrict attention to controllers of
the form
\begin{equation}
  U_t = g_t\bigl(\PXM tt\bigr),
\end{equation}
that is controller belonging to $\sG_S$, the family of functions from
$\P{\X\times\M}$ to $\RR^{d_U}$ that are
$\BOREL{\P{\X\times\M}}/\BOREL{\RR^{d_U}}$ measurable. Thus at each stage
we can optimize over a fixed (rather than a time varying) domain.

With this reduction, we can define information states $\pi^c_t, \pi^l_t,
\pi^g_t$ as in \autoref{def:info_states}, but the beliefs given by
\autoref{def:beliefs_uncountable}. These information states satisfy
\autoref{lemma:info_states}, and the proof follows the proof of
\autoref{lemma:info_states}; thus they are sufficient for performance
evaluation and lead to a sequential decomposition of the problem. An optimal
design can be obtained by the nested optimality
equations~\eqref{eq:DPbasic}--\eqref{eq:DPn}. Similar results extend to
infinite horizon problems using the ideas of \autoref{sec:infinite}.
 

Numerically these problems are not any harder than the problems with finite
state space; because of the following results from probability
theory~\cite[Appendix~1--5]{Dynkin:1975}:

\begin{definition}[Borel Space]
  A measurable space $B$ is called \emph{Borelian} or a \emph{Borel space} if
  it is isomorphic to a measurable subset of a Polish (i.e., a complete
  separable metric) space $E$.
\end{definition}

Consider the following Borel spaces
\begin{enumerate}
  \item A finite or countable space $S$, with the $\sigma$-algebra of all
    subsets.
  \item  The unit interval $I$ with the $\sigma$-algebra of all open
    subintervals.
\end{enumerate}

\begin{theorem}
  Every Borel space is isomorphic to either $S$ or to $I$.
\end{theorem}

\begin{theorem}\label{thm:probability}
  Suppose that $\P{E}$ is the set of all probability measures on he space
  $E$. If $E$ is a Borel space, then $\P{E}$ is also a Borel space.
\end{theorem}

For the finite state space problem, let $E$ denote the space $\X\times\M$
with $\sigma$-algebra $2^{\X\times\M}$; for the uncountable state space
problem, let $E$ denote the space $\RR^{d_X}\times\M$ with $\sigma$-algebra$
\BOREL {\RR^{d_X}}\times2^{\M}$. Then $E$ is Borelean and by \autoref{thm:probability}, the space
$\P{\X\times\M}$ of probability measures on $E$ is a Borel space. By the same
argument, the space $\Pi$ of probability measures on
$\bigl(E\times\P{E}, \BOREL{E\times\P{E}}\bigr)$ is a
Borel space. Thus the information state for the finite state space problem and
the information state for the infinite state space problem are isomorphic;
each being isomorphic to $I$, the unit interval with $\sigma$-algebra of all
open subintervals. The action space in both problems in uncountable. Thus, the
finite and uncountable state space problems have the same order of complexity.



